Recent advances in the evolution of interfaces: thermodynamics, upscaling, and universality

We consider the evolution of interfaces in binary mixtures permeating strongly heterogeneous systems such as porous media. To this end, we first review available thermodynamic formulations for binary mixtures based on \emph{general reversible-irreversible couplings} and the associated mathematical attempts to formulate a \emph{non-equilibrium variational principle} in which these non-equilibrium couplings can be identified as minimizers. Based on this, we investigate two microscopic binary mixture formulations fully resolving heterogeneous/perforated domains: (a) a flux-driven immiscible fluid formulation without fluid flow; (b) a momentum-driven formulation for quasi-static and incompressible velocity fields. In both cases we state two novel, reliably upscaled equations for binary mixtures/multiphase fluids in strongly heterogeneous systems by systematically taking thermodynamic features such as free energies into account as well as the system's heterogeneity defined on the microscale such as geometry and materials (e.g. wetting properties). In the context of (a), we unravel a \emph{universality} with respect to the coarsening rate due to its independence of the system's heterogeneity, i.e. the well-known ${\cal O}(t^{1/3})$-behaviour for homogeneous systems holds also for perforated domains. Finally, the versatility of phase field equations and their \emph{thermodynamic foundation} relying on free energies, make the collected recent developments here highly promising for scientific, engineering and industrial applications for which we provide an example for lithium batteries.

==> coarsening.tex <==
The first systematic report on the radial dependence of the coarsening/repening process 
seems to go back to Ostwald in 1900. Since this ``Ostwald ripening'' happens in almost 
all phase transition processes and governs the morphology of microstructure, 
Ostwald's discovery of this competitive growth phenomenon plays a crucial role in 
materials science and related applications. 
An important property of the morphology is its self-similarity which one can observe 
after sufficiently long coarsening times. The physical explanation for the Ostwald 
ripening is that the system tries to minimize its energy by reducing the 
system's interfaical area. Moreover, coarsening relies on the fact that a single 
large particle has much lower interfacial area than many small particles. 
We note that this ripening/coarsening appears in different characteristic length 
scales such as distance between particles, particle radius, or the inverse of the 
interfacial area per volume, i.e., $L(t) = \av{D}/E_{\rm mix}$, where 
$\frac{1}{\av{D}}E_{\rm mix}$ 
is the volume-averaged interfacial area which relies on the Cahn-Hilliard 
free energy density $f_{\rm mix}$, see \reff{E_mix}. 
We note that the Cahn-Hilliard equation associated with 
$\reff{E_mix}$ is a simple formulation for first order phase transitions. 




==> coarseningComp.tex <==
% !TeX root = interfacialev.tex
\pgfplotsset{width=7cm,compat=1.3}

\begin{tikzpicture}
	\begin{loglogaxis}[legend pos=north west]%[clickable coords={Level \thisrow{level} (q=\thisrow{q})}]
%
% Square with L=0.05 and alpha=3.3333
	\addplot table[y=t,x=L] {
%level  dof     error           q      
%1      4       2.50000000e-01  48        
%2      16      6.25000000e-02  25        
%3      64      1.56250000e-02  41        
%4      256     3.90625000e-03  8         
%5      1024    9.76562500e-04  22        
%6      4096    2.44140625e-04  46        
%7      16384   6.10351562e-05  40        
%8      65536   1.52587891e-05  3
%9      262144  3.81469727e-06  1
%10     1048576 9.53674316e-07  9
t L 3rdRoot
0.00311108090114 1e-06 0.0001
0.00311372757274 2.1e-05 0.000275892417638
0.00326418494763 4.1e-05 0.000344821724038
0.00526540293172 6.1e-05 0.00039364971831
0.00636675507901 8.1e-05 0.000432674871092
0.00686248176422 0.000101 0.00046570095078
0.00725948565118 0.000121 0.000494608744325
0.00756057231477 0.000141 0.000520482786339
0.00783703252659 0.000161 0.000544012182541
0.00821957188763 0.000181 0.000565665282582
0.0086156052786 0.000201 0.000585776600265
0.00884115740221 0.000221 0.000604594359601
0.00901632390888 0.000241 0.000622308425321
0.00916697517903 0.000261 0.00063906765284
0.00946705728582 0.000281 0.000654991162012
0.00981317614521 0.000301 0.000670175939538
0.0101649015503 0.000321 0.000684702127757
0.0105669694399 0.000341 0.000698636802782
0.0108503897881 0.000361 0.00071203673589
0.0110287875809 0.000381 0.000724950452421
0.0111862860271 0.000401 0.000737419794016
0.0113361884842 0.000421 0.000749481122586
0.0114801094194 0.000441 0.000761166261102
0.01160695255 0.000461 0.000772503237978
0.0117116570906 0.000481 0.000783516882696
0.0118955823869 0.000501 0.000794229307304
0.0121664405556 0.000521 0.000804660299297
0.0123464790603 0.000541 0.000814827644936
0.0125129934223 0.000561 0.000824747397412
0.0127249732185 0.000581 0.000834434100888
0.0128992834603 0.000601 0.000843900978927
0.0131421963203 0.000621 0.000853160093955
0.0133909911481 0.000641 0.000862222483005
0.0137096492654 0.000661 0.000871098273871
0.0138883562357 0.000681 0.000879796785032
0.0139765618511 0.000701 0.000888326611993
0.0140372695089 0.000721 0.000896695702239
0.0140882545403 0.000741 0.00090491142057
0.0141409100625 0.000761 0.000912980606272
0.01421973812 0.000781 0.000920909623339
0.0142929061199 0.000801 0.000928704404738
0.0143621598858 0.000821 0.000936370491556
0.0144330295741 0.000841 0.000943913067739
0.0145004758913 0.000861 0.000951336990991
0.0145599829112 0.000881 0.000958646820357
0.0146131230576 0.000901 0.000965846840908
0.014672798162 0.000921 0.000972941085875
0.0147649180539 0.000941 0.000979933356568
0.014877911569 0.000961 0.000986827240322
0.015022355378 0.000981 0.000993626126722
0.0151449184282 0.001001 0.00100033322228
0.0152380973857 0.001021 0.00100695156378
0.0153115636324 0.001041 0.00101348403037
0.0156073419577 0.001061 0.00101993335461
0.0159069963101 0.001081 0.00102630213253
0.01607275894 0.001101 0.00103259283287
0.0161766192833 0.001121 0.00103880780546
0.0162518680052 0.001141 0.00104494928899
0.0163237443786 0.001161 0.00105101941812
0.016412549288 0.001181 0.00105702022996
	};
% Ellipse with L=2.5 and alpha=4.0
\addplot table[x=t,y=L] {
L t
0.00311245818041 1e-06
0.00311412622032 2.1e-05
0.00320841706118 4.1e-05
0.00499075814993 6.1e-05
0.0063830813942 8.1e-05
0.00688813015104 0.000101
0.00725818920117 0.000121
0.00761885577858 0.000141
0.00793801682941 0.000161
0.00827502748559 0.000181
0.00857739994546 0.000201
0.00880062344751 0.000221
0.00910427981976 0.000241
0.00931164574777 0.000261
0.00942458096197 0.000281
0.00957014186041 0.000301
0.00968835272166 0.000321
0.00990503885284 0.000341
0.010204572524 0.000361
0.0104414226826 0.000381
0.010716653942 0.000401
0.0110689067176 0.000421
0.0113138827399 0.000441
0.0114535531856 0.000461
0.0117183932284 0.000481
0.0120327446873 0.000501
0.0122614700693 0.000521
0.0124328549692 0.000541
0.012626047893 0.000561
0.0128236032042 0.000581
0.0130055767101 0.000601
0.013152243501 0.000621
0.0132807320363 0.000641
0.0134228753364 0.000661
0.0135559102791 0.000681
0.0136692815177 0.000701
0.0137604137575 0.000721
0.0138315800294 0.000741
0.0138842026282 0.000761
0.0139217794933 0.000781
0.0139601835138 0.000801
0.0140329020336 0.000821
0.0141373393501 0.000841
0.0143283858908 0.000861
0.0145428164876 0.000881
0.0147387186123 0.000901
0.0149069534828 0.000921
0.0150763894822 0.000941
0.0152436495083 0.000961
0.0153846489424 0.000981
0.0154991803727 0.001001
0.0155982945681 0.001021
0.0156894461243 0.001041
0.0157749750218 0.001061
0.0158515563034 0.001081
0.0159153701568 0.001101
0.0159701903142 0.001121
0.0160211941665 0.001141
0.0160686694595 0.001161
0.016111546359 0.001181
	};
%
% Ellipse with L=2.5 and alpha=4.0
\addplot table[x=t,y=cube_t] {
L t cube_t 
0.00311245818041 1e-06 0.001
0.00311412622032 2.1e-05 0.00275892417638
0.00320841706118 4.1e-05 0.00344821724038
0.00499075814993 6.1e-05 0.0039364971831
0.0063830813942 8.1e-05 0.00432674871092
0.00688813015104 0.000101 0.0046570095078
0.00725818920117 0.000121 0.00494608744325
0.00761885577858 0.000141 0.00520482786339
0.00793801682941 0.000161 0.00544012182541
0.00827502748559 0.000181 0.00565665282582
0.00857739994546 0.000201 0.00585776600265
0.00880062344751 0.000221 0.00604594359601
0.00910427981976 0.000241 0.00622308425321
0.00931164574777 0.000261 0.0063906765284
0.00942458096197 0.000281 0.00654991162012
0.00957014186041 0.000301 0.00670175939538
0.00968835272166 0.000321 0.00684702127757
0.00990503885284 0.000341 0.00698636802782
0.010204572524 0.000361 0.0071203673589
0.0104414226826 0.000381 0.00724950452421
0.010716653942 0.000401 0.00737419794016
0.0110689067176 0.000421 0.00749481122586
0.0113138827399 0.000441 0.00761166261102
0.0114535531856 0.000461 0.00772503237978
0.0117183932284 0.000481 0.00783516882696
0.0120327446873 0.000501 0.00794229307304
0.0122614700693 0.000521 0.00804660299297
0.0124328549692 0.000541 0.00814827644936
0.012626047893 0.000561 0.00824747397412
0.0128236032042 0.000581 0.00834434100888
0.0130055767101 0.000601 0.00843900978927
0.013152243501 0.000621 0.00853160093955
0.0132807320363 0.000641 0.00862222483005
0.0134228753364 0.000661 0.00871098273871
0.0135559102791 0.000681 0.00879796785032
0.0136692815177 0.000701 0.00888326611993
0.0137604137575 0.000721 0.00896695702239
0.0138315800294 0.000741 0.0090491142057
0.0138842026282 0.000761 0.00912980606272
0.0139217794933 0.000781 0.00920909623339
0.0139601835138 0.000801 0.00928704404738
0.0140329020336 0.000821 0.00936370491556
0.0141373393501 0.000841 0.00943913067739
0.0143283858908 0.000861 0.00951336990991
0.0145428164876 0.000881 0.00958646820357
0.0147387186123 0.000901 0.00965846840908
0.0149069534828 0.000921 0.00972941085875
0.0150763894822 0.000941 0.00979933356568
0.0152436495083 0.000961 0.00986827240322
0.0153846489424 0.000981 0.00993626126722
0.0154991803727 0.001001 0.0100033322228
0.0155982945681 0.001021 0.0100695156378
0.0156894461243 0.001041 0.0101348403037
0.0157749750218 0.001061 0.0101993335461
0.0158515563034 0.001081 0.0102630213253
0.0159153701568 0.001101 0.0103259283287
0.0159701903142 0.001121 0.0103880780546
0.0160211941665 0.001141 0.0104494928899
0.0160686694595 0.001161 0.0105101941812
0.016111546359 0.001181 0.0105702022996
	};
\legend{square, ellipse, $t^{-1/3}$};
	\end{loglogaxis}
\end{tikzpicture}
\hfill

